LipsFormer: Introducing Lipschitz Continuity to Vision Transformers

We present a Lipschitz continuous Transformer, called LipsFormer, to pursue training stability both theoretically and empirically for Transformer-based models. In contrast to previous practical tricks that address training instability by learning rate warmup, layer normalization, attention formulation, and weight initialization, we show that Lipschitz continuity is a more essential property to ensure training stability. In LipsFormer, we replace unstable Transformer component modules with Lipschitz continuous counterparts: CenterNorm instead of LayerNorm, spectral initialization instead of Xavier initialization, scaled cosine similarity attention instead of dot-product attention, and weighted residual shortcut. We prove that these introduced modules are Lipschitz continuous and derive an upper bound on the Lipschitz constant of LipsFormer. Our experiments show that LipsFormer allows stable training of deep Transformer architectures without the need of careful learning rate tuning such as warmup, yielding a faster convergence and better generalization. As a result, on the ImageNet 1K dataset, LipsFormer-Swin-Tiny based on Swin Transformer training for 300 epochs can obtain 82.7\% without any learning rate warmup. Moreover, LipsFormer-CSwin-Tiny, based on CSwin, training for 300 epochs achieves a top-1 accuracy of 83.5\% with 4.7G FLOPs and 24M parameters. The code will be released at \url{https://github.com/IDEA-Research/LipsFormer}.

==> LipsFormer_Arxiv 2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> LipsFormer_Arxiv 2/mkdown.tex <==

General Reply:


We would like to thank all the reviewers for their valuable and constructive comments. 

To address reviewers' comments and concerns, we have made the following changes:

* We clarify our theoretical and empirical contributions more clearly with newly added experiments in Sec. K. 

* We add more experimental results of LipsFormer on ImageNet-v2, ImageNet-R and ImageNet-A in Sec. E.
    
* We further apply LipsFormer components on Swin-Transformer, which we call LipsFormer-Swin. We conduct extensive experiments on LipsFormer-Swin with varying model sizes: from Tiny (~ 30M) to Large++ (> 500M) in Sec. D. 

* We add figures showing how the learnable parameters change during training, as well as training curves in Sec. F and Sec. G.
    
* We add an experimental comparison between the scaled cosine similarity attention and L2 self-attention. We also further clarify the theoretical difference between them in Sec. H.
    
We mark the revised content in blue color for your reference. 















To R1:


We thank the reviewer for the constructive suggestions (and happy to know that you enjoy reading our work). We have added more experimental results according to your comments.

\
&nbsp;


### Response to your key concern and our improvements
_"Your main concern is whether the LipsFormer can stablely generalize to large model (e.g., >300M)"_

**Our response**: in the rebuttal stage, we apply LipsFormer components on Swin Transformer (named LipsFormer-Swin), and conduct extensive experiments on LipsFormer-Swin of different model sizes from Tiny (31 M), to Small (52M), Base (96M), Large (214M) and Large++ (526M) training on ImageNet-1K. We summarize our findings as below.

* All LipsFormer-Swin models, **_without_** any warmup, can stablely and successfully converge with competitive performance. We provide training curve of the largest model (LipsFormer-Swin Large++) in the revised paper. 


* Large model needs large scale data to avoid overfitting. 
We train our Tiny, Small, Base, Large and Large++ models on ImageNet-1K and already observe that LipsFormer-Swin-Large shows obvious overfitting (the training loss is smaller, but the test accuracy is lower) on ImageNet-1K. Similarly as discussed in github
[github issue](https://github.com/microsoft/Swin-Transformer/issues/261), it has also been observed that the original Swin-L cannot outperform Swin-B when training ONLY on ImageNet-1K. In our experiment, the LipsFormer-Swin Large++ can be smoothly trained on ImageNet-1K _without_ any learning rate warmup in spite of some overfitting.

\
&nbsp;



### Response to Clarity, Quality, Novelty and Reproducibility

**Our response**: thank your very much for your encouraging comments. We plan to release our code after it is accepted for publication.

\
&nbsp;

### Response to Summary Review
_You mention ``This paper provides several modules to control the Lipschitz constant of the Transformer models. The modules are theoretically justified and show promising numerical performance in ImageNet-K classification. It would be better if we could see the experiments on the large model (e.g., > 300M parameters).''}_
    
**Our response**: we train a LipsFormer-Swin-Large++ (526M) model on ImageNet-1K _without_ any learning rate warmup. The training process is smooth in spite of some overfitting. We hope this will address your concerns.


\
&nbsp;

### About Minor Issue

**Our response**: Thanks for pointing these out. We now add definition of the $\odot$ operator and a reference to Droppath in the main paper. 














To R2:




We thank the reviewer for the helpful suggestions (and happy to see that you like this new idea). We have revised our paper according to your comments. 

&nbsp;

## Response to your key concern and our improvements


* _"You suggest reporting the performance on more downstream tasks like object detection or semantic segmentation."_
    
**Our response**: in the revised paper, we apply our LipsFormer components on Swin-Transformer (named LipsFormer-Swin). We evaluate different versions (Tiny, Small, Base, Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained smoothly _without_ any warmup. Meanwhile, we add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. Apologies for not finishing experiments on more new tasks due to the limited time. We plan to include more downstream tasks in the future. 
    
&nbsp;

* _"You suggest adding more references for comparison."_
    
**Our response**: we now include your suggested works for comparison in the revised version. Thank you for your valuable comments. 
    
&nbsp;
* _"You suggest adding more metrics of computational cost to better understand the trade-offs."_
    
**Our response**: we now report our training costs, including training FPS and memory consumption in the revised paper. 
    
&nbsp;
* _"You suggest performing evaluation on more data sets."_
    
**Our response**: thank you for the valuable suggestions. We now add evaluations on two new datasets, including ImageNet-v2 and ImageNet-Real. The results are shown below. 


|Mode| Params (M) | Flops (G) | val | real| v2 |
| ------ |:------:|:------:|:------:|:------:|:------:|
| ViT-S | 22.0 | 4.6  | 80.4 | 86.1 | 69.7 |
| PiT-S | 23.5 | 2.9 | 80.4 | 86.1 | 69.2| 
| TNT-S | 23.8 | 5.2 | 81.4 | 87.2 | 70.6| 
| ConViT-S | 27.8 | 5.8 | 81.3 | 87.0 | 70.3| 
| Swin-S  | 49.6 | 8.7 | 82.1 | 86.9 | 70.7| 
| LipsFormer-CSwin-T |  24 | 4.7 | 83.5 | 88.0|  73.2| 
| ViT-B | 86.6 | 17.6|  83.1 | 87.7|  72.6| 
| PiT-B | 73.8|  12.5|  82.4|  86.8|  72.0| 
| TNT-B | 65.6|  14.1|  82.9|  87.6 | 72.2| 
| ConViT-B | 86.5 | 17.5 | 82.0 | 86.7|  71.3| 
| Swin-B | 87.8|  15.4 | 82.2 | 86.7 | 70.7| 
| CaiT-B12 | 100.0 | 18.2|  83.3|  87.7|  73.3| 
| LipsFormer-CSwin-B | 83|  16.3 | 84.6|  88.6|  74.5| 
    
\
&nbsp;

## Response to Summary Review
* _You mention "In general, I lean to positive and like this new idea. However, I have several concerns about the insufficient experiments. I hope this issue can be addressed in the next round."_
    
**Our response**: We now include more experiments according to your suggestion: 
* We apply our LipsFormer components on Swin-Transformer for a LipsFormer-Swin network. We evaluate different versions (Tiny, Small, Base and Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained stablely with competitive results.  
* We add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. Apologies for not finishing experiments on more new tasks due to the limited time. We plan to include more downstream tasks in the future.  

    
Hope the new experimental results would address your concerns.















To R3:









Thank you very much for your encouraging review and constructive suggestions. We have added more experiments and revised the paper according to your comments. We would like to provide  detailed responses for your questions.

&nbsp;

### Response to your key concern and our improvements


_"You ask whether the proposed CenterNorm that removes std(y) in the denominator will cause other issues due to ``covariate shift'' of neurons from different layers?"_
    
**Our response**:  Shibani \etal provided an intriguing perspective in their paper [1] that BatchNorm helps optimization not because it relieves ``covariate shift'' problem, but that _"We demonstrate that such distributional stability of layer inputs has little to do with the success of BatchNorm. Instead, we uncover a more fundamental impact of BatchNorm on the training process: it makes the optimization landscape significantly smoother."_ Lipschitz continuity with bounded Lipschitz constant also aims to encourage a smoother function and subsequently a smoother optimization landscape. 
    
In vision Transformers, given an input feature map y of shape $B\times H\times W\times C$, the statistics of Std(y) for each channel in BatchNorm is usually conducted on $B\times H \times W$, while the statistics of Std(y) for LayerNorm is usually conducted on $C$ only. Since $C$ is of much lower dimension than  $B\times H\times W$, Std(y) for LayerNorm is more prone to abnormal (high variance) std value, leading to a non-smooth landscape with high probability. Our proposed CenterNorm is a smoothed version of Normalization that has bounded Lipschitz constant.
        

&nbsp;

_"You suggest adding  comparison with the L2 self-attention, either theoretical and empirical comparison would be fine."_
    
**Our response**: thank you very much for the suggestion. We have added experimental comparison with L2 self-attention and clarified our theoretical differences. 

**Theoretically.**
For the L2 self-attention (L2SA), to **guarantee** its Lipschitz continuity, one **necessary condition** is $W_Q = W_K$ as proved in the original L2 self-attention paper.
    
For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$
where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized.

Our SCSA **_puts no constraints_** on $W_Q$, $W_K$ and $W_V$. We have clarified this point more clearly in the revised paper.

**Empirically.** We conduct experiments to compare L2 self-attention with our SCSA, as well as the original dot-product attention. 



| Attention  | Acc. |
| ------------- |:-------------:|
| Dot Product      | Diverged   |
| L2 Distance Attn      | 81.3     |
| SCSA      |81.6   |


Besides your suggested experiments, we also add more experiments on large models in the revised paper. 

&nbsp;    
    
_"You suggest providing how learnable parameters (e.g., $\boldsymbol{\alpha}$) change during training."_
    
**Our response**: thank you for your helpful suggestion. We now add a figure to show how $\boldsymbol{\alpha}$ changes during training. Meanwhile, we also provide the training curve of our model for more clarity on the training process. 
    

\
&nbsp;

### Response to Clarity, Quality, Novelty And Reproducibility

_"You suggest ``It would be better to also give the dimension of the input, output and weight matrices. For instance, the definition of Layer Normalization is for $\mathbf{x} \in \mathbb{R}^{D}$, and the equation will look different when the input is a high dimensional tensor."_
    
**Our response**: we have revised the paper according to your comments. 

\
&nbsp;

### Response to Summary Review
We have supplied more experimental results and comparisons. Thank you for all the helpful suggestions.

&nbsp;

[1] Santurkar, Shibani, Dimitris Tsipras, Andrew Ilyas, and Aleksander Madry. "How does batch normalization help optimization?." Advances in Neural Information Processing Systems 31 (2018).














To R4




Thank you very much for your valuable and constructive suggestions. We have provided more experiments, further clarified our theoretical and empirical contributions and revised the paper according to your comments. We provide detailed responses for each weakness you kindly pointed out, hopefully to address your concerns.

\
&nbsp;

### Response to your key concern and our improvements


_"You suggest applying LipsFormer on other baseline vision transformer."_
    
**Our response**: in the revised paper, we have applied our LipsFormer components on Swin-Transformer for a new LipsFormer-Swin network. We evaluate different versions (Tiny, Small, Base and Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained stablely (thanks to the Lipschitz properties) with competitive results. Meanwhile, we also add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. 
    
&nbsp;

_"You suggest adding training curves in the paper."_
    
**Our response**: thank you very much for the suggestion, we have added some related training curves including loss and training accuracy along with the training epoch in Figure 4 in the revised paper. 
    
&nbsp;

_"You suggest adding theoretical and empirical comparison with L2 self-attention."_

**Our response**: thank you very much for the suggestion. We have added experimental comparison with L2 self-attention and clarified our theoretical differences. 

**Theoretically.**
For the L2 self-attention (L2SA), to **guarantee** its Lipschitz continuity, one **necessary condition** is $W_Q = W_K$ as proved in the original L2 self-attention paper.
    
For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$
where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized.

Our SCSA **_puts no constraints_** on $W_Q$, $W_K$ and $W_V$. We have clarified this point more clearly in the revised paper.

**Empirically.** We conduct experiments to compare L2 self-attention with our SCSA, as well as the original dot-product attention. 



| Attention  | Acc. |
| ------------- |:-------------:|
| Dot Product      | Diverged   |
| L2 Distance Attn      | 81.3     |
| SCSA      |81.6   |


Besides your suggested experiments, we also add more experiments on large models in the revised paper. 

&nbsp;    
    
















_"You mention that ``In both Scaled Cosine Similarity Attention and Weighted Residual Shortcut, the predefined or learnable parameters can be absorbed into the weights, $W^{Q}, W^{K}, W^{V}$ or $W$, to recover the standard dot-product attention and residual connection. Also, the Weighted Residual Shortcut has been explored in [2]. Thus, these two components are not novel."_
    
**Our response**: thank you very much for the comment. We would like to argue that from the perspective of optimization, for both Scaled Cosine Similarity Attention and Weighted Residual Shortcut, the predefined or learnable parameters \textbf{cannot} be absorbed into the weights. 
    
For the Weighted Residual Shortcut (WRS),
    

$$
    \operatorname{WRS}(\boldsymbol{x}, \boldsymbol{W}) = \boldsymbol{x} + \boldsymbol{\alpha} \odot f(\boldsymbol{x}, \boldsymbol{W}),
$$
the learnable parameters $\boldsymbol{\alpha}$ cannot be absorbed into a matrix because the current WRS adopts a reparameterization trick that is widely used in deep learning optimization. The optimization problem, when the reparameterization trick is applied, is different from the absorbed version. A classical example of the reparameterization trick (similar to our formulation) is Weight Normalization [1], 
$$\mathbf{w}=g \frac{\mathbf{v}}{\|\mathbf{v}\|},$$

$\text { where } \mathbf{v} \text { is a}  \text { vector, } g \text { is a scalar, and }\|\mathbf{v}\| \text { denotes the Euclidean norm of } \mathbf{v}.$ In the equation, $\mathbf{w}$ is reparameterized into two terms $g$ and $\mathbf{v}$.
When formulated with two disentangled terms, each term would be individually optimized, inducing a different optimization process. 
One more example of the reparameterization trick  is  as shown in variational Bayesian inference [2]. Therefore, the learnable parameters in Weighted Residual Shortcut cannot be absorbed into the weights.

For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$

where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized: \\ $\mathbf{q}_i, \mathbf{k}_i, \mathbf{v}_i = \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{Q})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{Q} \|}^2 + \epsilon}}, \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{K})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{K} \|}^2 + \epsilon}}, \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{V})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{V} \|}^2 + \epsilon}}$;
    
the *non-linear transformation* of the cosine similarity in SCSA makes the parameters absorbing not equivalent to our original definition of SCSA. Therefore, the optimization is different between our original SCSA and the suggested absorbed version.  












    

\
&nbsp;

### Response to Additional Concerns and Questions

_"You mention ``Compared to the baseline CSwin Transformer, the LipsFormer has more parameters and more FLOPs. I am not sure if the advantage of LipsFormer over the baseline CSwin Transformer is from the Lipschitz continuity or just because the LipsFormer has a larger size and does more computation."_
    
**Our response**: The number of parameters for CSwin and LipsFormer-CSwin are 23M and 24M respectively, and the corresponding FLOPs are 4.3G and 4.7G. The increases are arguably negligible. 
     
&nbsp;    

_"You ask is there any result to support that the value of the weight of a residual shortcut decided by the network depth is better than other values?"_
    
**Our response**: Our choice of a residual shortcut weight decided by the network depth is inspired by Lipschitz constraint. Apologies that we do not yet have standalone experiment verifying its effectiveness against other random choices. But we do give a theoretical derivation of the Lipschitz constant of the LipsFormer network based on our Lipschitz continuity assumption of the network and validated the assumption by extensive experiments. 
    

\
&nbsp;

### Response to Summary Review
_You mention "I have two major concerns. First, the proposed Lipschitz continuous components are not novel. Second, there is a significant lack of experimental results to validate the advantage of LipsFormer."_
    
**Our response**: thank you very much for your comments, we have provided more experimental results in the revised paper according to your suggestion. We would like to clarify our contributions more clearly from both theoretical and empirical perspectives. 
    
**Theoretically.**

* We introduce a Lipschitz continuous attention and derive a theoretical Lipschitz constant upper bound for scaled cosine similarity attention. Meanwhile, we give a thorough Lipschitz analysis of key Transformer components: LayerNorm, self-attention, residual shortcut, and weight initialization. We believe these are valuable contributions towards a more stable vision transformer network.

* We propose a Lipschitz continuous Transformer (LipsFormer), and derive a theoretical Lipschitz constant upper bound for LipsFormer. The derivation provides a principled guidance for designing transformer networks that are easier to train (more stable).  

    
**Empirically.**

* We make an assumption about the Lipschitz continuity of LipsFormer, and experimentally validated that LipsFormer exhibits good training properties such as more stable training (even \emph{without} warmup) and better classification accuracy. 
    
* We evaluate LipsFormer designs on  Swin-Transformer and CSwin. We validate the efficacy of the the resultant networks of different sizes (Tiny, Small, Base and Large) of LipsFormer-Swin and LipsFormer-CSwin on ImageNet, ImageNet-v2, ImageNet-R datasets showing competitive results. 

Hope our clarifications could address your concerns. 



[1] Salimans, Tim, and Durk P. Kingma. "Weight normalization: A simple reparameterization to accelerate training of deep neural networks." Advances in neural information processing systems 29 (2016).

[2] Kingma, Durk P., Tim Salimans, and Max Welling. "Variational dropout and the local reparameterization trick." Advances in neural information processing systems 28 (2015).


==> LipsFormer_Arxiv 2/reply_again.tex <==
We thank the reviewer for the quick reply, which is very helpful for us. We would be happy to address any additional concerns.



**Our response to Q1**: Apologies for not making the purpose of Table 8 more clear. As detailed in Section E, Table 8 is an overfitting evaluation as suggested by reviewer C9zf. As pointed out by previous work [1,2], testing how a method performs in a nearby setting without any finetuning is a good way to assess overfitting. The evaluation is to see how our method, that works well on the original ImageNet validation set, performs on two additional data sets (ImageNet-real and ImageNet-v2). For example, 


|Mode| Params (M) | Flops (G) | val | real| v2 |
| ------ |:------:|:------:|:------:|:------:|:------:|
| CaiT-B12 | 100.0 | 18.2|  83.3|  87.7|  73.3| 
| LipsFormer-CSwin-B | 83|  16.3 | 84.6|  88.6|  74.5| 

According to the above table, the gap between CaiT-B12 and LipsFormer-CSwin-B is 1.3% on ImageNet-val, and the gap on ImageNet-v2 is 1.2\%. It shows that our method does not overfit to the ImageNet validation set.


&nbsp;


**Our response to Q2**: thank you very much for your question. To address your concern, we would like to provide analyses from two aspects.

First, we decrease the model size of LipsFormer to be the same as Swin Transformer for performance comparison. For Swin-T, it has [2,2,6,2] blocks in four stages, we use [2,2,5,2] for our LipsFormer-Swin-T to ensure the models have the same number of parameters. The results are shown below,

|Model | Params (M) | Flops (G) | Blocks | Acc. |
| ------ |:------:|:------:|:------:|:------:|
| Swin-T | 29 | 4.5 | [2,2,6,2]| 81.2|  
| LipsFormer-Swin-T | 29|  4.5 | [2,2,5,2]|  82.4 | 

We can see that LipsFormer-Swin-T still shows superior performance.

Second, we would like to list some relevant works to get a grasp on how the number of the parameters affect model performance.


|Model | Params (M) | Flops (G)  | Acc. |
| ------ |:------:|:------:|:------:|
| Swin-T | 29 | 4.5 | 81.2|  
|Twins-PCPVT-B [3] | 43.8  |  6.7 | 82.7 |
| LipsFormer-Swin-T | 31|  4.9 | 82.7 | 

It's obvious that LipsFormer improvements bring significant increase in performance with only mild increase in parameters and Flops.



&nbsp;

**Our response to Q3**: thank you very much for your suggestion. We will include it in the new revision. Meanwhile, we would like to point out the following observations: 1). Swin Transformer cannot be trained **_without learning rate warmup_** due to Nan or Exploding; 2). Our LipsFormer **_can_** be trained stably without learning rate warmup. This observation validates that good Lipschitz continuity of a network can make the training stabilized without training stabilization tricks such as learning rate warmup.

&nbsp;

**Our response to Q4**: This is a very good question and the short answer is no. In fact, L2 distance attention uses the same number of parameters as SCSA, including weight matrices $W^Q, W^K, W^V$ and a temperature $\tau$ (a scalar).

As proved in the paper [4], to ensure Lipschitz continuity of L2 distance attention, it is required that $W^Q = W^K$. However, enforcing $W^Q = W^K$ limits the expressiveness of the L2 distance attention resulting in inferior performance, extensive ablation study was conducted in the paper for this point. Therefore, in practice, they do not rigorously enforce the equality of $W^Q$ and $W^K$.




[1] Touvron, Hugo, Andrea Vedaldi, Matthijs Douze, and Hervé Jégou. "Fixing the train-test resolution discrepancy." Advances in Neural Information Processing Systems 32 (2019).

[2] Touvron, Hugo, Matthieu Cord, and Hervé Jégou. "Deit iii: Revenge of the vit." arXiv preprint arXiv:2204.07118 (2022).

[3] Chu, Xiangxiang, Zhi Tian, Yuqing Wang, Bo Zhang, Haibing Ren, Xiaolin Wei, Huaxia Xia, and Chunhua Shen. "Twins: Revisiting the design of spatial attention in vision transformers." Advances in Neural Information Processing Systems 34 (2021): 9355-9366.

[4] Kim, Hyunjik, George Papamakarios, and Andriy Mnih. "The lipschitz constant of self-attention." In International Conference on Machine Learning, pp. 5562-5571. PMLR, 2021.


==> mkdown.tex <==

General Reply:


We would like to thank all the reviewers for their valuable and constructive comments. 

To address reviewers' comments and concerns, we have made the following changes:

* We clarify our theoretical and empirical contributions more clearly with newly added experiments in Sec. K. 

* We add more experimental results of LipsFormer on ImageNet-v2, ImageNet-R and ImageNet-A in Sec. E.
    
* We further apply LipsFormer components on Swin-Transformer, which we call LipsFormer-Swin. We conduct extensive experiments on LipsFormer-Swin with varying model sizes: from Tiny (~ 30M) to Large++ (> 500M) in Sec. D. 

* We add figures showing how the learnable parameters change during training, as well as training curves in Sec. F and Sec. G.
    
* We add an experimental comparison between the scaled cosine similarity attention and L2 self-attention. We also further clarify the theoretical difference between them in Sec. H.
    
We mark the revised content in blue color for your reference. 















To R1:


We thank the reviewer for the constructive suggestions (and happy to know that you enjoy reading our work). We have added more experimental results according to your comments.

\
&nbsp;


### Response to your key concern and our improvements
_"Your main concern is whether the LipsFormer can stablely generalize to large model (e.g., >300M)"_

**Our response**: in the rebuttal stage, we apply LipsFormer components on Swin Transformer (named LipsFormer-Swin), and conduct extensive experiments on LipsFormer-Swin of different model sizes from Tiny (31 M), to Small (52M), Base (96M), Large (214M) and Large++ (526M) training on ImageNet-1K. We summarize our findings as below.

* All LipsFormer-Swin models, **_without_** any warmup, can stablely and successfully converge with competitive performance. We provide training curve of the largest model (LipsFormer-Swin Large++) in the revised paper. 


* Large model needs large scale data to avoid overfitting. 
We train our Tiny, Small, Base, Large and Large++ models on ImageNet-1K and already observe that LipsFormer-Swin-Large shows obvious overfitting (the training loss is smaller, but the test accuracy is lower) on ImageNet-1K. Similarly as discussed in github
[github issue](https://github.com/microsoft/Swin-Transformer/issues/261), it has also been observed that the original Swin-L cannot outperform Swin-B when training ONLY on ImageNet-1K. In our experiment, the LipsFormer-Swin Large++ can be smoothly trained on ImageNet-1K _without_ any learning rate warmup in spite of some overfitting.

\
&nbsp;



### Response to Clarity, Quality, Novelty and Reproducibility

**Our response**: thank your very much for your encouraging comments. We plan to release our code after it is accepted for publication.

\
&nbsp;

### Response to Summary Review
_You mention ``This paper provides several modules to control the Lipschitz constant of the Transformer models. The modules are theoretically justified and show promising numerical performance in ImageNet-K classification. It would be better if we could see the experiments on the large model (e.g., > 300M parameters).''}_
    
**Our response**: we train a LipsFormer-Swin-Large++ (526M) model on ImageNet-1K _without_ any learning rate warmup. The training process is smooth in spite of some overfitting. We hope this will address your concerns.


\
&nbsp;

### About Minor Issue

**Our response**: Thanks for pointing these out. We now add definition of the $\odot$ operator and a reference to Droppath in the main paper. 














To R2:




We thank the reviewer for the helpful suggestions (and happy to see that you like this new idea). We have revised our paper according to your comments. 

&nbsp;

## Response to your key concern and our improvements


* _"You suggest reporting the performance on more downstream tasks like object detection or semantic segmentation."_
    
**Our response**: in the revised paper, we apply our LipsFormer components on Swin-Transformer (named LipsFormer-Swin). We evaluate different versions (Tiny, Small, Base, Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained smoothly _without_ any warmup. Meanwhile, we add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. Apologies for not finishing experiments on more new tasks due to the limited time. We plan to include more downstream tasks in the future. 
    
&nbsp;

* _"You suggest adding more references for comparison."_
    
**Our response**: we now include your suggested works for comparison in the revised version. Thank you for your valuable comments. 
    
&nbsp;
* _"You suggest adding more metrics of computational cost to better understand the trade-offs."_
    
**Our response**: we now report our training costs, including training FPS and memory consumption in the revised paper. 
    
&nbsp;
* _"You suggest performing evaluation on more data sets."_
    
**Our response**: thank you for the valuable suggestions. We now add evaluations on two new datasets, including ImageNet-v2 and ImageNet-Real. The results are shown below. 


|Mode| Params (M) | Flops (G) | val | real| v2 |
| ------ |:------:|:------:|:------:|:------:|:------:|
| ViT-S | 22.0 | 4.6  | 80.4 | 86.1 | 69.7 |
| PiT-S | 23.5 | 2.9 | 80.4 | 86.1 | 69.2| 
| TNT-S | 23.8 | 5.2 | 81.4 | 87.2 | 70.6| 
| ConViT-S | 27.8 | 5.8 | 81.3 | 87.0 | 70.3| 
| Swin-S  | 49.6 | 8.7 | 82.1 | 86.9 | 70.7| 
| LipsFormer-CSwin-T |  24 | 4.7 | 83.5 | 88.0|  73.2| 
| ViT-B | 86.6 | 17.6|  83.1 | 87.7|  72.6| 
| PiT-B | 73.8|  12.5|  82.4|  86.8|  72.0| 
| TNT-B | 65.6|  14.1|  82.9|  87.6 | 72.2| 
| ConViT-B | 86.5 | 17.5 | 82.0 | 86.7|  71.3| 
| Swin-B | 87.8|  15.4 | 82.2 | 86.7 | 70.7| 
| CaiT-B12 | 100.0 | 18.2|  83.3|  87.7|  73.3| 
| LipsFormer-CSwin-B | 83|  16.3 | 84.6|  88.6|  74.5| 
    
\
&nbsp;

## Response to Summary Review
* _You mention "In general, I lean to positive and like this new idea. However, I have several concerns about the insufficient experiments. I hope this issue can be addressed in the next round."_
    
**Our response**: We now include more experiments according to your suggestion: 
* We apply our LipsFormer components on Swin-Transformer for a LipsFormer-Swin network. We evaluate different versions (Tiny, Small, Base and Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained stablely with competitive results.  
* We add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. Apologies for not finishing experiments on more new tasks due to the limited time. We plan to include more downstream tasks in the future.  

    
Hope the new experimental results would address your concerns.















To R3:









Thank you very much for your encouraging review and constructive suggestions. We have added more experiments and revised the paper according to your comments. We would like to provide  detailed responses for your questions.

&nbsp;

### Response to your key concern and our improvements


_"You ask whether the proposed CenterNorm that removes std(y) in the denominator will cause other issues due to ``covariate shift'' of neurons from different layers?"_
    
**Our response**:  Shibani \etal provided an intriguing perspective in their paper [1] that BatchNorm helps optimization not because it relieves ``covariate shift'' problem, but that _"We demonstrate that such distributional stability of layer inputs has little to do with the success of BatchNorm. Instead, we uncover a more fundamental impact of BatchNorm on the training process: it makes the optimization landscape significantly smoother."_ Lipschitz continuity with bounded Lipschitz constant also aims to encourage a smoother function and subsequently a smoother optimization landscape. 
    
In vision Transformers, given an input feature map y of shape $B\times H\times W\times C$, the statistics of Std(y) for each channel in BatchNorm is usually conducted on $B\times H \times W$, while the statistics of Std(y) for LayerNorm is usually conducted on $C$ only. Since $C$ is of much lower dimension than  $B\times H\times W$, Std(y) for LayerNorm is more prone to abnormal (high variance) std value, leading to a non-smooth landscape with high probability. Our proposed CenterNorm is a smoothed version of Normalization that has bounded Lipschitz constant.
        

&nbsp;

_"You suggest adding  comparison with the L2 self-attention, either theoretical and empirical comparison would be fine."_
    
**Our response**: thank you very much for the suggestion. We have added experimental comparison with L2 self-attention and clarified our theoretical differences. 

**Theoretically.**
For the L2 self-attention (L2SA), to **guarantee** its Lipschitz continuity, one **necessary condition** is $W_Q = W_K$ as proved in the original L2 self-attention paper.
    
For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$
where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized.

Our SCSA **_puts no constraints_** on $W_Q$, $W_K$ and $W_V$. We have clarified this point more clearly in the revised paper.

**Empirically.** We conduct experiments to compare L2 self-attention with our SCSA, as well as the original dot-product attention. 



| Attention  | Acc. |
| ------------- |:-------------:|
| Dot Product      | Diverged   |
| L2 Distance Attn      | 81.3     |
| SCSA      |81.6   |


Besides your suggested experiments, we also add more experiments on large models in the revised paper. 

&nbsp;    
    
_"You suggest providing how learnable parameters (e.g., $\boldsymbol{\alpha}$) change during training."_
    
**Our response**: thank you for your helpful suggestion. We now add a figure to show how $\boldsymbol{\alpha}$ changes during training. Meanwhile, we also provide the training curve of our model for more clarity on the training process. 
    

\
&nbsp;

### Response to Clarity, Quality, Novelty And Reproducibility

_"You suggest ``It would be better to also give the dimension of the input, output and weight matrices. For instance, the definition of Layer Normalization is for $\mathbf{x} \in \mathbb{R}^{D}$, and the equation will look different when the input is a high dimensional tensor."_
    
**Our response**: we have revised the paper according to your comments. 

\
&nbsp;

### Response to Summary Review
We have supplied more experimental results and comparisons. Thank you for all the helpful suggestions.

&nbsp;

[1] Santurkar, Shibani, Dimitris Tsipras, Andrew Ilyas, and Aleksander Madry. "How does batch normalization help optimization?." Advances in Neural Information Processing Systems 31 (2018).














To R4




Thank you very much for your valuable and constructive suggestions. We have provided more experiments, further clarified our theoretical and empirical contributions and revised the paper according to your comments. We provide detailed responses for each weakness you kindly pointed out, hopefully to address your concerns.

\
&nbsp;

### Response to your key concern and our improvements


_"You suggest applying LipsFormer on other baseline vision transformer."_
    
**Our response**: in the revised paper, we have applied our LipsFormer components on Swin-Transformer for a new LipsFormer-Swin network. We evaluate different versions (Tiny, Small, Base and Large) of LipsFormer-Swin training on ImageNet-1K, and show that all models can be trained stablely (thanks to the Lipschitz properties) with competitive results. Meanwhile, we also add more evaluations of our LipsFormer on ImageNet-v2 and ImageNet-Real datasets. 
    
&nbsp;

_"You suggest adding training curves in the paper."_
    
**Our response**: thank you very much for the suggestion, we have added some related training curves including loss and training accuracy along with the training epoch in Figure 4 in the revised paper. 
    
&nbsp;

_"You suggest adding theoretical and empirical comparison with L2 self-attention."_

**Our response**: thank you very much for the suggestion. We have added experimental comparison with L2 self-attention and clarified our theoretical differences. 

**Theoretically.**
For the L2 self-attention (L2SA), to **guarantee** its Lipschitz continuity, one **necessary condition** is $W_Q = W_K$ as proved in the original L2 self-attention paper.
    
For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$
where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized.

Our SCSA **_puts no constraints_** on $W_Q$, $W_K$ and $W_V$. We have clarified this point more clearly in the revised paper.

**Empirically.** We conduct experiments to compare L2 self-attention with our SCSA, as well as the original dot-product attention. 



| Attention  | Acc. |
| ------------- |:-------------:|
| Dot Product      | Diverged   |
| L2 Distance Attn      | 81.3     |
| SCSA      |81.6   |


Besides your suggested experiments, we also add more experiments on large models in the revised paper. 

&nbsp;    
    
















_"You mention that ``In both Scaled Cosine Similarity Attention and Weighted Residual Shortcut, the predefined or learnable parameters can be absorbed into the weights, $W^{Q}, W^{K}, W^{V}$ or $W$, to recover the standard dot-product attention and residual connection. Also, the Weighted Residual Shortcut has been explored in [2]. Thus, these two components are not novel."_
    
**Our response**: thank you very much for the comment. We would like to argue that from the perspective of optimization, for both Scaled Cosine Similarity Attention and Weighted Residual Shortcut, the predefined or learnable parameters \textbf{cannot} be absorbed into the weights. 
    
For the Weighted Residual Shortcut (WRS),
    

$$
    \operatorname{WRS}(\boldsymbol{x}, \boldsymbol{W}) = \boldsymbol{x} + \boldsymbol{\alpha} \odot f(\boldsymbol{x}, \boldsymbol{W}),
$$
the learnable parameters $\boldsymbol{\alpha}$ cannot be absorbed into a matrix because the current WRS adopts a reparameterization trick that is widely used in deep learning optimization. The optimization problem, when the reparameterization trick is applied, is different from the absorbed version. A classical example of the reparameterization trick (similar to our formulation) is Weight Normalization [1], 
$$\mathbf{w}=g \frac{\mathbf{v}}{\|\mathbf{v}\|},$$

$\text { where } \mathbf{v} \text { is a}  \text { vector, } g \text { is a scalar, and }\|\mathbf{v}\| \text { denotes the Euclidean norm of } \mathbf{v}.$ In the equation, $\mathbf{w}$ is reparameterized into two terms $g$ and $\mathbf{v}$.
When formulated with two disentangled terms, each term would be individually optimized, inducing a different optimization process. 
One more example of the reparameterization trick  is  as shown in variational Bayesian inference [2]. Therefore, the learnable parameters in Weighted Residual Shortcut cannot be absorbed into the weights.

For the Scaled Cosine Similarity Attention (SCSA), 
$$
\operatorname{SCSA}(\boldsymbol{X}, \boldsymbol{W}^{Q}, \boldsymbol{W}^{K}, \boldsymbol{W}^{V}, \nu, \tau) =  \nu \boldsymbol{P} \boldsymbol{V}, 
\text{where } 
\boldsymbol{P} = \operatorname{softmax}\left(\tau \boldsymbol{Q} \boldsymbol{K}^{\top} \right), 
$$

where $\nu$ and $\tau$ are predefined or learnable scalars; $\boldsymbol{Q}, \boldsymbol{K}, \boldsymbol{V}$ are $\ell^2$ row-normalized: \\ $\mathbf{q}_i, \mathbf{k}_i, \mathbf{v}_i = \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{Q})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{Q} \|}^2 + \epsilon}}, \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{K})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{K} \|}^2 + \epsilon}}, \frac{{({\mathbf{x}_i}^{\top} \boldsymbol{W}^{V})}^{\top}}{\sqrt{{\|{\mathbf{x}_i}^{\top} \boldsymbol{W}^{V} \|}^2 + \epsilon}}$;
    
the *non-linear transformation* of the cosine similarity in SCSA makes the parameters absorbing not equivalent to our original definition of SCSA. Therefore, the optimization is different between our original SCSA and the suggested absorbed version.  












    

\
&nbsp;

### Response to Additional Concerns and Questions

_"You mention ``Compared to the baseline CSwin Transformer, the LipsFormer has more parameters and more FLOPs. I am not sure if the advantage of LipsFormer over the baseline CSwin Transformer is from the Lipschitz continuity or just because the LipsFormer has a larger size and does more computation."_
    
**Our response**: The number of parameters for CSwin and LipsFormer-CSwin are 23M and 24M respectively, and the corresponding FLOPs are 4.3G and 4.7G. The increases are arguably negligible. 
     
&nbsp;    

_"You ask is there any result to support that the value of the weight of a residual shortcut decided by the network depth is better than other values?"_
    
**Our response**: Our choice of a residual shortcut weight decided by the network depth is inspired by Lipschitz constraint. Apologies that we do not yet have standalone experiment verifying its effectiveness against other random choices. But we do give a theoretical derivation of the Lipschitz constant of the LipsFormer network based on our Lipschitz continuity assumption of the network and validated the assumption by extensive experiments. 
    

\
&nbsp;

### Response to Summary Review
_You mention "I have two major concerns. First, the proposed Lipschitz continuous components are not novel. Second, there is a significant lack of experimental results to validate the advantage of LipsFormer."_
    
**Our response**: thank you very much for your comments, we have provided more experimental results in the revised paper according to your suggestion. We would like to clarify our contributions more clearly from both theoretical and empirical perspectives. 
    
**Theoretically.**

* We introduce a Lipschitz continuous attention and derive a theoretical Lipschitz constant upper bound for scaled cosine similarity attention. Meanwhile, we give a thorough Lipschitz analysis of key Transformer components: LayerNorm, self-attention, residual shortcut, and weight initialization. We believe these are valuable contributions towards a more stable vision transformer network.

* We propose a Lipschitz continuous Transformer (LipsFormer), and derive a theoretical Lipschitz constant upper bound for LipsFormer. The derivation provides a principled guidance for designing transformer networks that are easier to train (more stable).  

    
**Empirically.**

* We make an assumption about the Lipschitz continuity of LipsFormer, and experimentally validated that LipsFormer exhibits good training properties such as more stable training (even \emph{without} warmup) and better classification accuracy. 
    
* We evaluate LipsFormer designs on  Swin-Transformer and CSwin. We validate the efficacy of the the resultant networks of different sizes (Tiny, Small, Base and Large) of LipsFormer-Swin and LipsFormer-CSwin on ImageNet, ImageNet-v2, ImageNet-R datasets showing competitive results. 

Hope our clarifications could address your concerns. 



[1] Salimans, Tim, and Durk P. Kingma. "Weight normalization: A simple reparameterization to accelerate training of deep neural networks." Advances in neural information processing systems 29 (2016).

[2] Kingma, Durk P., Tim Salimans, and Max Welling. "Variational dropout and the local reparameterization trick." Advances in neural information processing systems 28 (2015).


==> reply_again.tex <==
We thank the reviewer for the quick reply, which is very helpful for us. We would be happy to address any additional concerns.



**Our response to Q1**: Apologies for not making the purpose of Table 8 more clear. As detailed in Section E, Table 8 is an overfitting evaluation as suggested by reviewer C9zf. As pointed out by previous work [1,2], testing how a method performs in a nearby setting without any finetuning is a good way to assess overfitting. The evaluation is to see how our method, that works well on the original ImageNet validation set, performs on two additional data sets (ImageNet-real and ImageNet-v2). For example, 


|Mode| Params (M) | Flops (G) | val | real| v2 |
| ------ |:------:|:------:|:------:|:------:|:------:|
| CaiT-B12 | 100.0 | 18.2|  83.3|  87.7|  73.3| 
| LipsFormer-CSwin-B | 83|  16.3 | 84.6|  88.6|  74.5| 

According to the above table, the gap between CaiT-B12 and LipsFormer-CSwin-B is 1.3% on ImageNet-val, and the gap on ImageNet-v2 is 1.2\%. It shows that our method does not overfit to the ImageNet validation set.


&nbsp;


**Our response to Q2**: thank you very much for your question. To address your concern, we would like to provide analyses from two aspects.

First, we decrease the model size of LipsFormer to be the same as Swin Transformer for performance comparison. For Swin-T, it has [2,2,6,2] blocks in four stages, we use [2,2,5,2] for our LipsFormer-Swin-T to ensure the models have the same number of parameters. The results are shown below,

|Model | Params (M) | Flops (G) | Blocks | Acc. |
| ------ |:------:|:------:|:------:|:------:|
| Swin-T | 29 | 4.5 | [2,2,6,2]| 81.2|  
| LipsFormer-Swin-T | 29|  4.5 | [2,2,5,2]|  82.4 | 

We can see that LipsFormer-Swin-T still shows superior performance.

Second, we would like to list some relevant works to get a grasp on how the number of the parameters affect model performance.


|Model | Params (M) | Flops (G)  | Acc. |
| ------ |:------:|:------:|:------:|
| Swin-T | 29 | 4.5 | 81.2|  
|Twins-PCPVT-B [3] | 43.8  |  6.7 | 82.7 |
| LipsFormer-Swin-T | 31|  4.9 | 82.7 | 

It's obvious that LipsFormer improvements bring significant increase in performance with only mild increase in parameters and Flops.



&nbsp;

**Our response to Q3**: thank you very much for your suggestion. We will include it in the new revision. Meanwhile, we would like to point out the following observations: 1). Swin Transformer cannot be trained **_without learning rate warmup_** due to Nan or Exploding; 2). Our LipsFormer **_can_** be trained stably without learning rate warmup. This observation validates that good Lipschitz continuity of a network can make the training stabilized without training stabilization tricks such as learning rate warmup.

&nbsp;

**Our response to Q4**: This is a very good question and the short answer is no. In fact, L2 distance attention uses the same number of parameters as SCSA, including weight matrices $W^Q, W^K, W^V$ and a temperature $\tau$ (a scalar).

As proved in the paper [4], to ensure Lipschitz continuity of L2 distance attention, it is required that $W^Q = W^K$. However, enforcing $W^Q = W^K$ limits the expressiveness of the L2 distance attention resulting in inferior performance, extensive ablation study was conducted in the paper for this point. Therefore, in practice, they do not rigorously enforce the equality of $W^Q$ and $W^K$.




[1] Touvron, Hugo, Andrea Vedaldi, Matthijs Douze, and Hervé Jégou. "Fixing the train-test resolution discrepancy." Advances in Neural Information Processing Systems 32 (2019).

[2] Touvron, Hugo, Matthieu Cord, and Hervé Jégou. "Deit iii: Revenge of the vit." arXiv preprint arXiv:2204.07118 (2022).

[3] Chu, Xiangxiang, Zhi Tian, Yuqing Wang, Bo Zhang, Haibing Ren, Xiaolin Wei, Huaxia Xia, and Chunhua Shen. "Twins: Revisiting the design of spatial attention in vision transformers." Advances in Neural Information Processing Systems 34 (2021): 9355-9366.

[4] Kim, Hyunjik, George Papamakarios, and Andriy Mnih. "The lipschitz constant of self-attention." In International Conference on Machine Learning, pp. 5562-5571. PMLR, 2021.

